An Incremental Singular Value Decomposition Approach for Large-Scale Spatially Parallel & Distributed but Temporally Serial Data -- Applied to Technical Flows

The paper presents a strategy to construct an incremental Singular Value Decomposition (SVD) for time-evolving, spatially 3D discrete data sets. A low memory access procedure for reducing and deploying the snapshot data is presented. Considered examples refer to Computational Fluid Dynamic (CFD) results extracted from unsteady flow simulations, which are computed spatially parallel using domain decomposition strategies. The framework addresses state of the art PDE-solvers dedicated to practical applications. Although the approach is applied to technical flows, it is applicable in similar applications under the umbrella of Computational Science and Engineering (CSE). To this end, we introduce a bunch matrix that allows the aggregation of multiple time steps and SVD updates, and significantly increases the computational efficiency. The incremental SVD strategy is initially verified and validated by simulating the 2D laminar single-phase flow around a circular cylinder. Subsequent studies analyze the proposed strategy for a 2D submerged hydrofoil located in turbulent two-phase flows. Attention is directed to the accuracy of the SVD-based reconstruction based on local and global flow quantities, their physical realizability, the independence of the domain partitioning, and related implementation aspects. Moreover, the influence of lower and (adaptive) upper construction rank thresholds on both the effort and the accuracy are assessed. The incremental SVD process is applied to analyze and compress the predicted flow field around a Kriso container ship in harmonic head waves at Fn = 0.26 and ReL = 1.4E+07. With a numerical overhead of O(10%), the snapshot matrix of size O(R10E+08 x 10E+04) computed on approximately 3000 processors can be incrementally compressed by O(95%). The storage reduction is accompanied by errors in integral force and local wave elevation quantities of O(1E-02%).

==> tex/old-Introduction_1_.tex <==
\section{Introduction}
Engineering computational methods are nowadays demanded to deliver more than the mere result of a performance analysis for a device exposed to particular operating conditions. In addition, the simulation results -- which often refer to several millions and more degrees of freedom (DoF) --  should also be exploitable for further problems that investigate different designs, different cost functions, and/or different operating conditions, preferably at a low computational cost.
 
When attention is directed to a few (integral) cost functions, aka. output parameters -- for example, the dynamic force on an object --  as a function of a few input parameters -- e.g., the angle of flow incidence of an airfoil %or a parameterized shape 
-- data-based machine learning (ML) approaches are nowadays intensively used to provide such input/output relations. Data-driven ML methods can estimate the cost functional (output) in response to formerly not explicitly investigated input parameters at a virtually negligible computational cost. However, they usually require the availability of a considerable body of data compiled by detailed first-principle simulations, e.g., transient, 3D fluid dynamic Navier-Stokes simulations. The latter are expensive due to the many degrees of freedom and yield substantial offline or background computing costs. 
%
As an alternative to ML strategies, physics-based reduced order models (ROMs) are employed to compress the information of detailed first-principle simulations into a rapidly analyzable form, using different variants of principle component analysis (PCA), aka. proper orthogonal decomposition (POD), singular value decomposition (SVD), or Karhunen-Lo\`eve Expansion-based projections, cf. \cite{benner2015survey, mainini2015surrogate}. ROM aims at extracting the physically dominant features or modes of the simulated fields, which are frequently limited to a few ten contributions.
%
Linearity assumptions somewhat restrict the use of ROM strategies. Nevertheless, the exponential convergence of ROM approximations is often recovered also in nonlinear fluid problems (e.g. \cite{lassila2014model}) due to the rapid decay in their Kolmogorov N-width, cf. \cite{kolmogoroff1936uber}. Hence, the solution manifold can be well approximated by a low-rank subspace. Thus, the linear POD (\cite{sirovich1987turbulence, kunisch2002galerkin, willcox2002balanced}) is still a leading tool in model order reduction of unsteady nonlinear Navier-Stokes systems. The framework was successfully applied to laminar (\cite{caiazzo2014numerical, stabile2018finite, grassle2019pod} as well as turbulent flow problems (\cite{wang2012proper, lorenzi2016pod, hijazi2020data}). Additionally, clear links  between ROM and ML approaches using convolutional neural network (CNN) methods exist for linear problems (\cite{murata2020nonlinear, agostini2020exploration}), which relate the reduced space of CNN auto-encoders to the modes of a ROM strategy. Therefore the application of hybrid ROM/ML strategies that blend data-based and physics-based information is currently receiving increasing attention \cite{benner2015survey, mainini2015surrogate, hesthaven2018non, swischuk2019projection, pache2022data}.
%
Numerous of the former techniques originate in a SVD, emphasizing the need for such techniques -- ideally incremental when addressing large-scale technical applications.
 
Typical applications of the compressed data refer to near-to-real-time extraction of output parameters entering decision support systems (\cite{walton2013reduced, mainini2015surrogate, pache2022data}) or field reconstructions for transient optimization studies (\cite{stoll2015low, dolgov2017low, vezyris2019incremental, buenger2020low, benner2020low, margetis2021lossy, margetis2022reducing}). Superficially, data compression strategies require the availability of the complete data to be compressed. However, the size of the spatio-temporal data sets generated by, for example, fluid dynamic simulation methods might involve O($10^7$) grid points and O($10^5$) time steps, and data handling can therefore be an issue. In such situations, data compression with modest computational overhead is of significance, i.e., using  (a) existing domain parallel High-Performance Computing (HPC) fragments and, at the same time (b) incrementally preparing the reduction in transient frameworks.
%
For instance, when attention is directed to the example of unsteady adjoint optimization methods, substantial computational expenses arise from the oppositely directed information transport of the primal and adjoint procedures. In a trade-off between compute and memory expenses, check-pointing strategies involve multiple storing and later re-reading, i.e., Input/Output (I/O), operations of complete fields at check points along the timeline and redundant forward integrations from the nearest check point to the current time step were previously suggested, cf. \cite{griewank1992achieving, griewank2000algorithm, symes2007reverse, wang2009minimal}. The related overheads often question their feasibility in an industrial design process and contradict the ever-growing effort to reduce the energy consumption of complex numerical simulations while adjusting the algorithm to the substantial performance gap between memory-intensive efforts (read, write) and compute-intensive efforts. In this regard, reduced order models are  more economical than repetitive forward integration(s) using possibly restricted time steps at lower memory requirements.

\subsubsection*{Objectives and Outline of the Paper}
The paper tries to convey a strategy to perform incremental order reduction methods for time-evolving, spatially partitioned 3D data sets. An --in terms of disk writing/reading effort-- effective procedure for archiving/compressing and later deploying procedurally distributed Partial Differential Equation (PDE)-related data (here, solution snapshots) is presented. Considered numerical studies refer to fluid dynamic data extracted from unsteady flow simulations, which are computed spatially parallel using domain decomposition strategies in combination with the Message Passing Interface (MPI) inter-processor communication protocol (\cite{mpi}). The spatial size of the data is assumed to be time-invariant and significantly larger than the temporal size due to the large computational mesh and the number of field quantities involved in practical simulations. Moreover, the paper highlights issues associated with large-scale simulations usually performed by spatially decomposing large data sets and employing distributed memory systems along the routes of a Single Instruction Multiple Data (SIMD) concept. Aspects relevant to practical success, such as, e.g., appropriate pre- and postconditioning, distributed data as well as matrix-vector structures, and incremental adaptivity aspects, are presented in detail. The overall procedure is grid type/structure independent.

Some theoretical aspects of this research have already been highlighted elsewhere, e.g., PDE solution tracking (\cite{fareed2018incremental, fareed2019note, fareed2020error}), low-rank PDE approximations (\cite{stoll2015low, buenger2020low, benner2020low}) or large-scale, partially distributed systems/networks (\cite{mastronardi2010fast, iwen2016distributed, lin2021low}). However, the previously published investigations did not address large systems and complex physics combinations. The latter poses particular challenges in terms of (a) the ROM construction (incrementally, computational, and storage efficiency) and (b) subsequent decomposition, e.g., as regards the physical realizability of reconstructed values, which are, for example, frequently addressed in established turbulence modeling strategies (\cite{schumann1977realizability, speziale1994realizability, rung1998realizability, heinz2020review}). Examples included herein refer to positive values of energy or concentration.

The remainder of the paper is organized as follows: Sec. \ref{sec:starting_point} outlines the algorithmic starting point and examines the paper's theoretical framework. Section \ref{sec:parallelization_aspects} translates the former into a spatially distributed but temporally serial framework, whereby several pseudo-codes should increase the comprehensibility of the algorithm's parallelization aspects. The governing physical equations, as well as basics about the employed fluid solver, are provided in Sec. \ref{sec:governing_equations}. Parallelization and accuracy aspects are studied on a generic laminar 2D circular cylinder's flow example in Sec. \ref{sec:verification_validation}. Subsequently, practical implementation and adaptivity issues are presented in Sec. \ref{sec:practical_issues} for the turbulent flow around a hydrofoil interacting with traveling water waves. Section \ref{sec:application} applies the former on a 3D container ship benchmark geometry exposed to regular head waves. Finally, conclusions are drawn in Sec. \ref{sec:conclusion_outlook}.

In the remainder of the paper, continuum mechanical field quantities are defined regarding Cartesian coordinates denoted by Latin subscripts, applying Einstein's summation convention to them. For example, $p$, $v_i$, and $S_{ik}$ represent the fluid dynamic scalar-valued pressure, vector-valued velocity, and matrix-valued shear rate field.
%
Moreover, vectors and matrices necessary in the paper's relevant algebraic operations are always written in lowercase and uppercase, respectively, and always in bold. For example, the matrix $\matr{A}$ is constructed by its column vectors $[\vect{a}_1, ..., \vect{a}_\mathrm{m}]$.


==> tex/old-Startingpoint_2_.tex <==
\section{Algorithmic Starting Point}
The concatenation of all $s = [1,...,\mathrm{S}]$ single state snapshot vectors $\vect{\varphi}$ of equal length $l = [1,...,\mathrm{L}]$, i.e., of an equal number of local discrete DoF, e.g., the number of control volumes, allows for the construction of a local total state snapshot vector $\vect{y}$ of length $\mathrm{Y} = \mathrm{S} \, \mathrm{L}$ at time $t \in [1, ..., \mathrm{T}]$ on partition (or processor, thread) $p \in [1, ..., \mathrm{P}]$, viz.
\begin{align}
    \vect{y}^{(t,p)} =
    \frac{1}{\mathrm{P} \, \mathrm{L}}
    \begin{bmatrix}
        \vect{\varphi}^\mathrm{(1,1:L,t,p)} \\
        \vdots \\
        \vect{\varphi}^\mathrm{(S,1:L,t,p)}
	\end{bmatrix}
	\qquad \qquad \mathrm{with} \qquad \qquad
    \vect{\varphi}^\mathrm{(s,1:L,t,p)} =
    \frac{1}{\varphi^\mathrm{ref}}
    \begin{bmatrix}  
		\varphi^\mathrm{(s,1,t,p)} \\
    	\vdots \\
	    \varphi^\mathrm{(s,L,t,p)} 
	\end{bmatrix} \, , \label{equ:SVD_start}
\end{align}
where $\varphi^\mathrm{ref}$ refers to a reference value per state that aims at (a) non-dimensionalization of the involved states that allows for their combination and (b) as a preconditioner that numerically harmonizes field variables that may arise in strongly varying magnitudes. For example, compare the fluid dynamics pressure of order $p = \mathcal{O}(10^5) \, \SI{}{Pa}$ with the velocity field of $v_i = \mathcal{O}(10^1) \, \SI{}{m/s}$.
%
In addition, all state vectors are divided by the constant number of discrete global DoF ($= \mathrm{P} \, \mathrm{L}$) to not shift later global matrix-vector products into ranges, possibly not representable, even in the context of double-precision arithmetics.
%
All (or selected) total state snapshot vectors per processor, aligned column by column, provide the following global state snapshot matrix that evolves in time
\begin{align}
    \matr{Y} = 
    \begin{bmatrix}
            \vect{y}^\mathrm{(1,1)} & \cdots    & \vect{y}^\mathrm{(T,1)}   \\
            \vdots                  &           & \vdots                    \\
            \vect{y}^\mathrm{(1,P)} & \cdots    & \vect{y}^\mathrm{(T,P)}
    \end{bmatrix} \label{equ:state_matrix}
\end{align}
of size $\matr{Y} \in \mathbb{R}^{(\mathrm{Y} \, \mathrm{P}) \times \mathrm{T}}$, where typically $\mathrm{Y} \, \mathrm{P} = (\mathrm{S} \, \mathrm{L}) \, \mathrm{P} >> \mathrm{T}$ holds, i.e., the solution of the considered problems are usually much more complex (elliptic) in space than in time and scale (non-linearly) with the number of field quantities.
%
For example, the maritime flow application shown later has $\mathrm{S} = 7$ field quantities with a spatial discretization of $\mathrm{L} \approx \SI{10000}{}$ discrete DoF on $\mathrm{P} = 2880$ partitions which are to be analyzed over a time horizon of $\mathrm{T} = \SI{20 000}{}$ time steps, yielding a global state matrix of approximately $\matr{Y} \in \mathbb{R}^{\SI{201 600 000}{} \times \SI{20 000}{}}$.
%
No doubt, it is practically impossible to store a matrix of this size, which is why simulation-based, resource-efficient singular value decomposition (SVD) techniques are presented for the outlined situation. The underlying tool refers to an incrementally constructed, truncated SVD as briefly derived in the following. Different variants of the SVD are presented, and relevant properties for this paper are summarized. The following statements are standard information and are reproduced for completeness and, above all, for the sake of understanding; their proofs are assumed to be known. 

\subsection{Singular Value Decomposition}
\label{subsec:svd}
Let $\matr{Y} \in \mathbb{R}^{\mathrm{N} \times \mathrm{M}}$, then there exist the orthogonal matrices $\matr{U} = \left( \vect{u}_1, ..., \vect{u}_\mathrm{N} \right) \in \mathbb{R}^{\mathrm{N} \times \mathrm{N}}$ and $\matr{V} = \left( \vect{v}_1, ..., \vect{v}_\mathrm{M} \right) \in \mathbb{R}^{\mathrm{M} \times \mathrm{M}}$ and a diagonal matrix $\matr{S} = \mathrm{diag}(s_\mathrm{i}) \in \mathbb{R}^{\mathrm{N} \times \mathrm{M}}$ such that
\begin{align}
    \matr{Y} = \matr{U} \matr{S} \matr{V}^T = \sum_{i=1}^d s_i \vect{u}_i \vect{v}_i^\mathrm{T} \label{equ:general_svd}
\end{align}
with unique singular values $s_1 \geq ... \geq s_\mathrm{d} \geq 0$, singular vectors $\vect{u}_\mathrm{i}, \vect{v}_\mathrm{j}$ and $d = \mathrm{min}(\mathrm{N}, \mathrm{M})$.
%
Note that the theoretical equality $\matr{Y} = \matr{U} \matr{S} \matr{V}^T$ holds only in the absence of numerical rounding errors, which is not feasible for practical applications with large matrices. Based on the preceding, two remarks of particular emphasis follow, which relate to the matrix $\matr{Y}$'s norm, viz.
\begin{align}
    ||\matr{Y}||_2 = s_1
    \qquad \qquad
    \mathrm{and}
    \qquad \qquad
    ||\matr{Y}||_\mathrm{F} = \sqrt{\sum_{i=1}^\mathrm{N} \sum_{i=1}^\mathrm{M} |y_\mathrm{ij}|^2} = \sqrt{\sum_{i=1}^d s_\mathrm{i}^2} \label{equ:norms} \, ,
\end{align}
where $||\cdot||_2$ and $||\cdot||_\mathrm{F}$ refer to the L2 and Frobenius norm, respectively. Additionally, let $r = \mathrm{max}(k \in \mathbb{N}: s_\mathrm{k} \neq 0)$ be the amount of non-zero singular values equivalent to $\mathrm{rank}(\matr{Y}) = r$. Hence, in line with Eqn. (\ref{equ:general_svd}) only the first $r$ singular vectors are needed to determine the matrix $\matr{Y}$ via the SVD, allowing for the following definition of a thin or reduced SVD (rSVD). Let $\mathrm{rank}(\matr{Y}) = r \leq \mathrm{min}(\mathrm{N},\mathrm{M})$ such that
\begin{align}
    \matr{Y} = \matr{U}_\mathrm{r} \matr{S}_\mathrm{r} \matr{V}_\mathrm{r}^\mathrm{T} = \sum_{i=1}^\mathrm{r} s_\mathrm{i} \vect{u}_\mathrm{i} \vect{v}_\mathrm{i}^\mathrm{T} \label{equ:reduced_svd}
\end{align}
where the rSVD matrices read $\matr{U}_\mathrm{r} = \left( \vect{u}_1, ..., \vect{u}_\mathrm{r} \right) \in \mathbb{R}^{\mathrm{N} \times \mathrm{r}}$ and $\matr{V}_\mathrm{r} = \left( \vect{v}_1, ..., \vect{v}_\mathrm{r} \right) \in \mathbb{R}^{\mathrm{M} \times \mathrm{r}}$ as well as $\matr{S}_\mathrm{r} = \mathrm{diag}(s_\mathrm{i}) \in \mathbb{R}^{\mathrm{r} \times \mathrm{r}}$. Note that instead of $\matr{Y}$, the matrices $\matr{U}_\mathrm{r}$ and $\matr{V}_\mathrm{r}$ and the vector of diagonal $\matr{S}$-entries $\vect{s} \in \mathbb{R}^\mathrm{r}$ have to be stored. In practice, this can result in a storage overhead since the matrix $\matr{Y}$ can be of high rank, although a steep decay in singular values is expected. 
%\nkuehl{Check if a SVD can be used for data compression}

Consequently, a further reduction is needed. Here, due to its broad applicability and versatility in linear and non-linear flow problems (\cite{lassila2014model}), a POD-based model-order reduction approach is pursued that provides a low-rank approximation while also preserving the overall solution behavior. Concerning the reduced SVD, this yields the approach of additionally truncating the smallest non-zero singular values up to a specific truncation criterion. This is consistent with the assumption of a fast decay in Kolmogorov N-width (\cite{kolmogoroff1936uber, benner2020model}), which is expressed as the POD modes corresponding to small singular values having only an insignificant impact on the approximation quality. This leads to the definition of a truncated SVD (tSVD). The rank-q tSVD of $\matr{Y}$ with $0 < q < r$ is defined as
\begin{align}
    \matr{Y}_\mathrm{q} = \matr{U}_\mathrm{q} \matr{S}_\mathrm{q} \matr{V}_\mathrm{q}^\mathrm{T} = \sum_\mathrm{i=1}^\mathrm{q} s_\mathrm{i} \vect{u}_\mathrm{i} \vect{v}_\mathrm{i}^\mathrm{T} \label{equ:truncated_svd}
\end{align}
with the tSVD matrices $\matr{U}_\mathrm{q} = \left( \vect{u}_1, ..., \vect{u}_\mathrm{q} \right) \in \mathbb{R}^{\mathrm{N} \times \mathrm{q}}$, $\matr{V}_\mathrm{q} = \left( \vect{v}_1, ..., \vect{v}_\mathrm{q} \right) \in \mathbb{R}^{\mathrm{M} \times \mathrm{q}}$ and $\matr{S}_\mathrm{q} = \mathrm{diag}(s_1, ..., s_\mathrm{q}) \in \mathbb{R}^{\mathrm{q} \times \mathrm{q}}$. $\matr{Y}_\mathrm{q} \in \mathbb{R}^{\mathrm{N} \times \mathrm{M}}$ denotes the matrix obtained by considering only the $q$ largest singular values of $\matr{Y}$ in its rSVD, cf. Eqn. (\ref{equ:reduced_svd}).

For the choice of the reduced order $q$, there is no clear way to determine it a-priori, i.e., before approximation start. The overall goal is almost always to choose a $q$ as small as possible and as large as necessary so that $\matr{Y}_\mathrm{q} \approx \matr{Y}$. The above truncation in terms of a tSVD raises the question of the impact of the truncation on the overall approximation quality. Although the obtained rank-$q$ approximation is optimal in the least-squared sense (\cite{eckart1936approximation}), this does not yield a clear path for rank determination. A widely used criterion to determine the quality of the truncation of the tSVD heuristically refers to the \textit{retained energy or information content $\eta^\mathrm{q}$} of the approximation, cf. \cite{grassle2018pod, gubisch2017proper, lassila2014model}. The latter has no physical, energetic character and is typically defined via the squared Frobenius norm (cf. Eqn. (\ref{equ:norms})) of the matrix $\matr{Y}$, viz. 
\begin{align}
    \eta^\mathrm{q}= \frac{||\matr{Y}_\mathrm{q}||_\mathrm{F}^2}{||\matr{Y}||_\mathrm{F}^2} = \frac{\sum_\mathrm{i=1}^\mathrm{q} s_\mathrm{i}^2}{\sum_\mathrm{i=1}^\mathrm{r} s_\mathrm{i}^2} = \frac{\sum_\mathrm{i=1}^\mathrm{q} s_\mathrm{i}^2}{\sum_\mathrm{i=1}^\mathrm{r} ||\vect{y}_\mathrm{i}||^2} \label{equ:retained_energy} \, .
\end{align}
Note that this quality criterion requires the totality of all $r$ singular values, which is impractical for large matrices of technical applications. However, in line with Eqn. (\ref{equ:norms}) and $d \to r$, one can alternatively compute $||\matr{Y}||_\mathrm{F}^2$ directly if the state snapshot vectors are -- at least once during the matrix construction or time integration -- available. This is the case in the temporally serial framework of this paper, i.e., $\sum_\mathrm{i=1}^\mathrm{r} ||\vect{y}_\mathrm{i}||^2$ can be computed exactly, i.e., with potential round-off but without any truncation error in an incremental fashion that will be considered in the upcoming section.
% 
Later studies in the application part of this paper will show that a minimal truncation rank $o$ is advantageous for adaptivity aspects. The reason for this is the partly extreme (numerical) dominance of the first singular values, which tend to drive the evaluation of the energetic bound in Eqn. (\ref{equ:retained_energy}) into the machine accuracy (consider that the singular values occur squared). Hence, the preceding energetic bound definition is adapted, which neglects the first $o$ singular values, viz.
\begin{align}
    \eta^\mathrm{o} = \frac{\sum_\mathrm{i=o}^\mathrm{q} s_\mathrm{i}^2}{\sum_\mathrm{i=o}^\mathrm{T} s_\mathrm{i}^2} = \frac{\sum_\mathrm{i=o}^\mathrm{q} s_\mathrm{i}^2}{\sum_\mathrm{i=o}^\mathrm{T} ||\vect{y}_\mathrm{i}||^2 - \sum_\mathrm{i=1}^\mathrm{o-1} s_\mathrm{i}^2} \label{equ:adaptive_energy} \, .
\end{align}
Note that relation (\ref{equ:retained_energy}) is recovered for $o = 1$. Additionally, $r$ is dictated by the number of time steps for $N >> M = T$ in Eqn. \ref{equ:state_matrix}, i.e., $r \to T$ in Eqn. \ref{equ:adaptive_energy}. Since this adaptivity criterion contains the exact reference energy in the denominator, the latter is substracted by the --always available-- first singular values.

%However, this quality criterion requires the totality of all $r$ singular values, which is impractical for large matrices of technical applications. Therefore, it is assumed that only the first $l$ singular values are available for the approximation, so that $r \geq l \geq q$ is valid, and the rank $r$ is roughly available (e.g. via the maximum number of time steps used for the SVD). Hereby, the energetic quality criterion (\ref{equ:retained_energy}) is modified, so that an upper $\eta^\mathrm{u}$ and lower $\eta^\mathrm{l}$ energetic bound is defined, where $l$ refers to the amount of economically computable singular values, viz.
%\begin{align}
%    \eta^u = \frac{\sum_{i=1}^q s_i^2}{\sum_{i=1}^l s_i^2}
%    \qquad \qquad
%    \mathrm{and}
%    \qquad \qquad 
%    \eta^l = \frac{\sum_{i=1}^q s_i^2}{\sum_{i=1}^l s_i^2 + (r-l)s_l^2} \, , \label{equ:energy_bounds}
%\end{align}
%such that $\eta^l \leq \eta \leq \eta^u$ holds. Here, the \textit{non-maintained or neglected energy} is \hfischer{bounded by $\eta^\mathrm{n} = \sum_{i=l+1}^r s_i^2 \leq (r-l) s_l^2$ due to the descending order of singular values.} 
%optimistically estimated, viz. $\eta^\mathrm{n} = \sum_{i=l+1}^r s_i^2 \approx (r-l) s_l^2$. 
%Later studies in the application part of this paper will show that --next to a maximal (e.g. determinable) rank-- a minimal counterpart is advantageous for adaptivity aspects. The reason for this is the partly extreme (numerical) dominance of the first singular values, which tend to drive the evaluation of the energetic bounds in Eqn. (\ref{equ:energy_bounds}) into the machine accuracy (consider that the singular values occur squared). Hence, adaptive itSVD studies employ a minimum evaluation rank $l^\text{min}$ in addition to the maximum rank $l \to l^\text{max}$ introduced above. The preceding definition of the energetic bounds is adapted, viz.
%\begin{align}
%    \eta^u = \frac{\sum_{i=l^\text{min}}^q s_i^2}{\sum_{i=l^\text{min}}^{l^\text{max}} s_i^2}
%    \qquad \qquad
%    \mathrm{and}
%    \qquad \qquad 
%    \eta^l = \frac{\sum_{i=l^\text{min}}^q s_i^2}{\sum_{i=l^\text{min}}^{l^\text{max}} s_i^2 + (T - l^\text{max})s_{l^\text{max}}^2} \, , \label{equ:energy_bounds_adjusted}
%\end{align}
%Note that relation (\ref{equ:energy_bounds}) is recovered for $l^\text{min} = 1$. Additionally, $r$ is dictated by the number of time steps for $N >> M = T$, i.e. $r \to T$ in Eqn. \ref{equ:energy_bounds}. Whereas the upper energetic bound tends to the unit value $\eta^u \to 1$ for $q \to l^\mathrm{max}$, its lower companion can be well below one $\eta^l \leq 1$ and only reach $\eta^l \to \eta^u$ in the case of $(T - l^\text{max}) \to 0$. Since the latter does usually not apply, the following can be summarized: In addition to specifying the minimum evaluation barrier $l^\text{min}$ and the (possibly hardware-dependent) maximum truncation rank $l^\text{max}$, it is thus feasible to define either only an upper energetic bound $\tilde{\eta}^u$, only a lower barrier $\tilde{\eta}^l$, or a combination of both, and based on them adjust the tSVD rank q in such a way, that specific conditions like, e.g., $\eta^u \geq \tilde{\eta}^u$ or $\eta^l \geq \tilde{\eta}^l$ are met. Details in this regard are discussed further in Sec. \ref{sec:practical_issues}.

From the preceding it can be deduced that it it should be possible to approximate the global state matrix via a (r,t)SVD according to Eqn. (\ref{equ:general_svd}), (\ref{equ:reduced_svd}) or (\ref{equ:truncated_svd}). However, the global matrix must be available for a one-shot computation, which --for large scale applications-- is practically challenging, that motivates the upcoming on the fly construction. 

\subsection{Additive Modification of a Singular Value Decomposition}
\label{sec:additive_svd}
This section aims to derive an algorithm that enhances an already existing SVD without any additional knowledge about the computation of the underlying system matrix. This methodology can then be used to update the SVD incrementally. For this purpose, at first, a general approach of an additive rank-b modification of the rSVD, mainly developed by \cite{brand2002incremental, brand2006fast}, is presented.

For a given matrix $\matr{Y} \in \mathbb{R}^{\mathrm{N} \times \mathrm{M}}$, let $\matr{Y} = \matr{U} \matr{S} \matr{V}^\mathrm{T}$ be its rank-r rSVD. Further, let $\matr{B} \in \mathbb{R}^{\mathrm{N} \times \mathrm{b}}$ and $\matr{C} \in \mathbb{R}^{\mathrm{M} \times \mathrm{b}}$ be arbitrary matrices of rank $b$ that describe the desired modification of the system matrix. Then the rSVD of $\matr{Y} + \matr{B} \matr{C}^\mathrm{T} = \tilde{\matr{U}} \tilde{\matr{S}} \tilde{\matr{V}}^\mathrm{T}$ is given by the three updated SVD matrices
\begin{align}
    \tilde{\matr{V}} &= 
    \begin{bmatrix}
            \matr{V} & \matr{Q}_\mathrm{C}
    \end{bmatrix} \matr{V}^\prime \label{equ:update_V_full} \\
    \tilde{\matr{S}} &= \matr{S}^\prime \label{equ:update_S_full} \\
    \tilde{\matr{U}} &= 
    \begin{bmatrix}
            \matr{U} & \matr{Q}_\mathrm{B}
    \end{bmatrix} \matr{U}^\prime \label{equ:update_U_full} 
\end{align}
where $\matr{Q}_\mathrm{B} \matr{R}_\mathrm{B} = (\matr{I} - \matr{U}\matr{U}^\mathrm{T})\matr{B}$ and $ \matr{Q}_\mathrm{C} \matr{R}_\mathrm{C} = (\matr{I} - \matr{V}\matr{V}^\mathrm{T})\matr{C}$ follow from two QR decompositions, respectively. Additionally, $\matr{U}^\prime \matr{S}^\prime {\matr{V}^\prime}^\mathrm{T}$ follows from the rSVD of a matrix $\matr{K} \in \mathbb{R}^{\mathrm{(r+b)} \times \mathrm{(r+b)}}$ that reads
\begin{align}
    \matr{K} = 
    \begin{bmatrix}
            \matr{S} & \matr{0} \\ \matr{0} & \matr{0}
    \end{bmatrix}
    +
    \begin{bmatrix}
            \matr{U}^\mathrm{T} \matr{B} \\ \matr{R}_\mathrm{B}
    \end{bmatrix}
    \begin{bmatrix}
            \matr{V}^\mathrm{T} \matr{C} \\ \matr{R}_\mathrm{C}
    \end{bmatrix}^\mathrm{T} 
    \label{equ:matrix_K_general} \, .
\end{align}
%
The approach outlined above provides a variety of possibilities to modify the system matrix. For instance, in addition to updating and down-dating, individual values can be modified, or rows and columns can be exchanged, cf. \cite{brand2002incremental, brand2006fast}. The necessary QR decomposition employ, e.g., a modified Gram-Schmidt procedure, and the decomposition's resulting matrices have dimensions of $\matr{Q}_\mathrm{B} \in \mathbb{R}^{\mathrm{N} \times \mathrm{b}}, \matr{Q}_\mathrm{C} \in \mathbb{R}^{\mathrm{M} \times \mathrm{b}}$ and $\matr{R}_\mathrm{B}, \matr{R}_\mathrm{C} \in \mathbb{R}^{\mathrm{b} \times \mathrm{b}}$.
%
The additive modifications presented above result in a rank enhancement and, thus, a higher memory consumption. Since $\tilde{\matr{S}} = \matr{S}^\prime$ in Eqn. (\ref{equ:update_S_full}), the rank-q truncation of an additive rank-b modification can be achieved by truncating $\matr{K}$ of Eqn. (\ref{equ:matrix_K_general}), i.e.,
\begin{align}
    \tilde{\matr{V}}_\mathrm{q} &= 
    \begin{bmatrix}
            \matr{V} & \matr{Q}_\mathrm{C}
    \end{bmatrix} \matr{V}^\prime(:,1:q) \label{equ:update_V_truncated} \\
    \tilde{\matr{S}}_\mathrm{q} &= \matr{S}^\prime(1:q, 1:q) \label{equ:update_S_truncated} \\
    \tilde{\matr{U}}_\mathrm{q} &= 
    \begin{bmatrix}
            \matr{U} & \matr{Q}_\mathrm{B}
    \end{bmatrix} \matr{U}^\prime(:,1:q) \label{equ:update_U_truncated} \, .
\end{align}
%
However, in this work, the focus is on the update, i.e., column extension of the system matrix $\matr{Y}$ that can be deduced from the preceding. By setting $\matr{C} = \begin{bmatrix} \matr{0} & \matr{I} \end{bmatrix}^\mathrm{T}$, a column update via the matrix $\matr{B}$ is achieved by extending $\matr{Y}$ and $\matr{V}$ with $b$ additional zero columns such that $\begin{bmatrix} \matr{Y} & \matr{0} \end{bmatrix} = \matr{U} \matr{S} \begin{bmatrix} \matr{V} & \matr{0} \end{bmatrix}^\mathrm{T} \in \mathbb{R}^{N \times (M+b)}$. 
%\nkuehl{Note that in this case
% \begin{align}
%     \begin{bmatrix}
%             \matr{A} & \matr{B}
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%             \matr{A} & \matr{0}
%     \end{bmatrix}
%     +
%     \matr{B}
%     \begin{bmatrix}
%             \matr{0} & \matr{I}
%     \end{bmatrix}
%     =
%     \begin{bmatrix}
%             \matr{A} & \matr{0}
%     \end{bmatrix}
%     +\begin{bmatrix}
%             \matr{0} & \matr{B}
%     \end{bmatrix} \, ,
% \end{align}
%and 
Since $\matr{C}$ is always an augmented identity matrix, its QR decomposition follows a certain structure that allows simplifying the former rank-b modification, i.e., $\matr{Q}_\mathrm{C} = \matr{I}$ and $\matr{R}_\mathrm{C} = \matr{C}$. Additionally, the zero entries in $\matr{C} = \begin{bmatrix} \matr{0} & \matr{I} \end{bmatrix}^\mathrm{T}$ yield $\begin{bmatrix} \matr{V} & \matr{0} \end{bmatrix}^\mathrm{T} \matr{C} = \matr{0}$, so that the qSVD [rSVD] of $\matr{A} + \matr{B} \matr{C}^\mathrm{T} \approx \tilde{\matr{U}}_\mathrm{q} \tilde{\matr{S}}_\mathrm{q} \tilde{\matr{V}}^\mathrm{T}_\mathrm{q}$ [$= \tilde{\matr{U}} \tilde{\matr{S}} \tilde{\matr{V}}^\mathrm{T}$] from (\ref{equ:update_V_truncated})-(\ref{equ:update_U_truncated}) [(\ref{equ:update_V_full})-(\ref{equ:matrix_K_general})] is now given by
\begin{align}
    \tilde{\matr{V}}_\mathrm{q} &= 
    \begin{bmatrix}
            \matr{V} & \matr{0} \\
            \matr{0} & \matr{I}
    \end{bmatrix} \matr{V}^\prime(:,1:q) \label{equ:update_V_column} \\
    \tilde{\matr{S}}_\mathrm{q} &= \matr{S}^\prime(1:q,1:q) \label{equ:update_S_column} \\
    \tilde{\matr{U}}_\mathrm{q} &= 
    \begin{bmatrix}
            \matr{U} & \matr{Q}_\mathrm{B}
    \end{bmatrix} \matr{U}^\prime(:,1:q) \label{equ:update_U_column} \, ,
\end{align}
where $\matr{U}^\prime \matr{S}^\prime {\matr{V}^\prime}^\mathrm{T}$ denotes the rSVD of $\matr{K}$ with
\begin{align}
    \matr{K} = 
    \begin{bmatrix}
            \matr{S} & \matr{U}^\mathrm{T} \matr{B} \\ \matr{0} & \matr{R}_\mathrm{B}
    \end{bmatrix}
    %= \matr{U}^\prime \matr{S}^\prime {\matr{V}^\prime}^\mathrm{T} 
    \label{equ:matrix_K_column} \, .
\end{align}
%
Eqns. (\ref{equ:update_V_column})-(\ref{equ:matrix_K_column}) serve as the basis for the on-the-fly or incrementally computed tSVD (itSVD) in this paper.

\paragraph{To conclude in between} At each time step, the instantaneous state snapshot vector $\vect{y}$ is aligned as an additional column of the so-called bunch-matrix $\matr{B}$, and every $b$ time steps when $\matr{B}$ is filled, the latter is appended to the previous itSVD based on (\ref{equ:update_V_column}) - (\ref{equ:matrix_K_column}). Subsequently, $\matr{B}$ is emptied, and the process restarts. Hence, a trade-off between the bunch-size or column-size $b$ of $\matr{B}$, the overall itSVD construction time, and the consumed (possibly available) memory arises. Two limit cases are conceivable: (a) The number of columns of the bunch matrix reaches the number of maximum time steps ($b \to T$), which de-facto no longer corresponds to an incremental  tSVD. Instead, it refers to a classical, large one-shot SVD performed at the end of the simulation. In contrast, one may (b) transform the matrix $\matr{B}$ into a column vector ($b \to 1$) and expand the itSVD every time step. While option (a) mainly addresses the required memory, (b) concerns the simulation time. Hence, analogous to the truncation value $q$, it can be concluded that in most scenarios, the bunch matrix width $b$ should be chosen as large as possible and as small as necessary.
%
These aspects are primarily technical, influenced mainly by the underlying HPC hardware --e.g., maximum (random access) memory sizes or simulation times, etc.-- and discussed later in Sec. \ref{sec:verification_validation}.

\subsection{Evaluation of the parallel itSVD}
Once the itSVD has been completed, e.g., at the end of the time horizon of interest, each column --and thus an approximation of the reconstructed state vector $\tilde{\vect{\varphi}}(:) \approx \vect{\varphi}(:)$-- follows from the subsequent evaluation of the itSVD. For this purpose, relation (\ref{equ:SVD_start}) is twisted, offering an expression for the approximated local instantaneous snapshot vector $\tilde{\vect{\varphi}}^\mathrm{(s,1:L,t,p)}$ of state $s$ and length $L$ at time $t$ on processor $p$, viz.
\begin{align}
    \begin{bmatrix}  
		\tilde{\varphi}^\mathrm{(s,1,t,p)} \\
    	\vdots \\
	    \tilde{\varphi}^\mathrm{(s,L,t,p)} 
	\end{bmatrix}
	= \varphi^\mathrm{ref} \tilde{\vect{\varphi}}^\mathrm{(s,1:L,t,p)}
	\quad\mathrm{with} \quad
    \begin{bmatrix}
        \tilde{\vect{\varphi}}^\mathrm{(1,1:L,t,p)} \\
        \vdots \\
        \tilde{\vect{\varphi}}^\mathrm{(S,1:L,t,p)}
	\end{bmatrix} 
	= \left( \mathrm{P} \, \mathrm{L}\right)  \tilde{\vect{y}}^{(t,p)}(:) = \tilde{\matr{U}}_q(:,1:\tilde{q}) \tilde{\matr{S}}_q(1:\tilde{q},1:\tilde{q}) \tilde{\matr{V}}_q^\mathrm{T}(t,1:\tilde{q})  \, . \label{equ:SVD_end}
\end{align}
Note that the reference quantities applied during the reconstruction (\ref{equ:SVD_end}) process should match those of the construction (\ref{equ:SVD_start}) phase. The same holds for the constant factor concerning the overall DoF $\mathrm{P} \, \mathrm{L}$. Furthermore, another parameter $\tilde{q} \leq q$ was introduced, which determines the reconstruction rank and should match the construction rank $\tilde{q} \to q$ for an approximation as accurate as possible in terms of the itSVD. Nevertheless, in some situations, one may be interested in information of lower rank, e.g., if only the first $\tilde{q}$, particularly energy-rich modes, are of interest. In this case, the numerical costs of the matrix-vector multiplications to be performed in Eqn. (\ref{equ:SVD_end}) decrease. The choice of $\tilde{q}$ concerning the reconstruction quality (which varies from case to case), as well as the parallelization described next, is studied in detail in Sec. \ref{sec:verification_validation}.

To simplify the notation and to increase readability, the rest of the paper consistently assumes the construction of a rank-q itSVD so that the tilde marking and subscripts $\tilde{\matr{U}}_q \tilde{\matr{S}}_q \tilde{\matr{V}}_q^\mathrm{T} \to \matr{U} \matr{S} \matr{V}^\mathrm{T}$ in (\ref{equ:update_V_column})-(\ref{equ:update_U_column}) are no longer explicitly stated.

Finally, physical plausibility should be ensured by the itSVD evaluation. However, numerical inaccuracies or even inaccurate approximations, e.g., via a too-small construction/truncation rank $q$/$\tilde{q}$, may cause the reconstructed field not to satisfy fundamental principles and circumstances. These may include, e.g., boundary, far-field, or coupling conditions that are no longer met. In the case of inhomogeneous Dirichlet boundary conditions, e.g., the description of varying inflow conditions, a potential defect can be addressed by the introduction of lifting functions, cf. \cite{ballarin2016pod, nonino2021monolithic}. Therein, the non-homogeneous boundary values are subtracted from the single-state snapshots to provide homogenized companions. This naturally guarantees the fulfillment of the Dirichlet boundary conditions of the reconstructed single-state. However, issues concerning boundary conditions were of minor importance for the present research. Significantly more crucial are physically unrealistic reconstructed fields that might inhere, e.g., negative energies or volume concentrations, as shown in the application part of the paper, cf. Sec. \ref{sec:practical_issues}. 
%
Additionally, since the itSVD is composed of divergence free snapshots any reconstructed reduced solution is also divergence free, i.e., the continuity equation is automatically fulfilled , cf. \cite{quarteroni2014reduced, caiazzo2014numerical, ballarin2015supremizer}.
%\hfischer{However, in case of inhomogeneous Dirichlet boundary conditions, e.g. the description of an inflow condition, the defect can be addressed by the introduction of a lifting function (\cite{nonino2021monolithic, ballarin2016pod}). The non-homogeneous boundary values are substracted from the single state snapshots to provide homogenized snapshots.
%which is defined by also fulfilling the boundary condition.
%$l = g(t, \pmb{\mu})$.
%The lifting function is then subtracted from single state to provide homogenized state snapshots on which the reduction is conducted. 
%This naturally guarantees the fulfillment of the Dirichlet boundary conditions of the reconstructed single state.}


==> tex/old-abstract.tex <==
\begin{abstract}
The paper presents a strategy to construct an incremental Singular Value Decomposition (SVD) for time-evolving, spatially partitioned 3D data sets. An --in terms of disk writing/reading effort-- effective procedure for archiving/compressing and later deploying procedurally distributed Partial Differential Equation (PDE)-related data (here, solution snapshots) is proposed. Considered numerical studies refer to Computational Fluid Dynamic (CFD) data extracted from unsteady flow simulations, which are computed spatially parallel using domain decomposition strategies combined with the Message Passing Interface (MPI) inter-processor communication protocol. The presented framework addresses state of the art PDE-solvers, i.e., the spatial size of the required data is assumed to be time-invariant and significantly larger than the temporal size due to the large computational mesh and the number of field quantities involved in practical simulations. The overall procedure is transferable to other state-of-the-art fluid solvers \nkuehl{(e.g., OpenFOAM and its derivatives, Ansys Fluent/CFX, Siemens STAR CCM+, etc.)} and in general grid type/structure independent. Although the proposed approach is applied to technical flows, it is portable to CFD-adjacent applications under the umbrella of Computational Science and Engineering, e.g., Computational Structure Dynamics (CSD), Acoustics (CA), or Electrodynamics (CEM).

The research highlights issues associated with large-scale simulations usually performed by spatially decomposing large data sets and employing distributed memory systems along the routes of a Single Instruction Multiple Data (SIMD) concept. Aspects relevant to practical success, such as --among others-- appropriate pre- and postconditioning, matrix-vector structures, and incremental adaptivity aspects, are presented in detail. The introduction of a bunch matrix allows the aggregation of multiple time steps, which makes the incremental SVD update after each time step obsolete, resulting in a measurable increase in numerical efficiency. Finally, various pseudo-codes allow for traceability and reprogramming.

The incremental SVD strategy is extensively verified and validated on two-dimensional flows past a circular cylinder at $\mathrm{Re}_\mathrm{D} = 100$. Next to the quality of the results based on local and global flow quantities, particular attention is given to the influence of spatial partitioning and related implementation aspects. Eventually, reduced memory requirements in terms of a truncated SVD and the associated increased computation times are discussed.
%
Subsequent studies test the proposed strategy on a hydrofoil placed under traveling harmonic water waves at $\mathrm{Fn} = 0.62$ and $\mathrm{Re}_\mathrm{L} = 7.5 \cdot 10^5$ concerning process adaptivity and truncated SVD evaluation realizability. Introducing a minimum SVD construction rank improves the adaptive behavior, which can become numerically uncomfortable due to the dominance of the first singular values. In contrast, during the SVD evaluation process, inaccurate SVD reconstructions can violate fundamental physical constraints such as positive energies or volume concentrations and are, therefore, particularly considered.
%
Finally, the incremental SVD process is applied to analyze and compress the flow field around a Kriso container ship in harmonic head waves at $\mathrm{Fn} = 0.26$ and $\mathrm{Re}_\mathrm{L} = 1.4 \cdot 10^7$. With a numerical overhead of $\mathcal{O}(10\%)$, the snapshot matrix of size $\mathcal{O}(\mathbb{R}^{\SI{210 000 000}{} \times \SI{10 000}{}})$ can be compressed by $\mathcal{O}(95\%)$, and the massive reduction of storage effort is accompanied by errors in integral quantities (here: drag and lift coefficient) of $\mathcal{O}(10^{-2}\%)$. \nkuehl{Shift parts to conclusion}
\end{abstract}

==> tex/playground.tex <==
\begin{algorithm}
\caption{Additive column adding rank-b modification of a tSVD}
\label{alg:itSVD}
\begin{algorithmic}[1]
\Require $r \in \mathbb{N}$, $B \in \mathbb{R}^{ny \times b}$, $U \in \mathbb{R}^{ny \times k}$, $S \in \mathbb{R}^{k \times k}$, $V \in \mathbb{R}^{nt \times k}$
\Ensure
$k = \mathrm{size}(U,2)$, 
$b = \mathrm{size}(B,2)$,
$l = \mathrm{min}(r,k+b)$
\Comment{Particular relevant sizes}
\Ensure
$U_\mathrm{tmp} \in \mathbb{R}^{(k+b) \times (k+b)}$,
$S_\mathrm{tmp} \in \mathbb{R}^{(k+b)}$,
$V_\mathrm{tmp} \in \mathbb{R}^{(k+b) \times (k+b)}$
\Comment{SVD related Allocations}

\State $M = U^\mathrm{T} B$                 \Comment{$M \in \mathbb{R}^{k \times b}$, Local}
\State parallel-sum($M$)                    \Comment{Local to Global}
\\
\State $P = B - U M$                        \Comment{$P \in \mathbb{R}^{ny \times b}$, Local}
\State $\tilde{P} = \mathrm{GramSchmidt}(P)$       \Comment{$\tilde{P} \in \mathbb{R}^{ny \times b}$, Global Orthonormalization (Alg. TBA)}
\\
\State $T = \tilde{P}^\mathrm{T} P$     \Comment{$T \in \mathbb{R}^{b,b}$, Local}
\State parallel-sum($T$)                   \Comment{Local to Global}
\\

\If{onmaster}   \Comment{SVD on master proc only}
    \State $K = \begin{bmatrix}
            S & 0 \\
            0 & T
    \end{bmatrix}$ \Comment{Prepare Local SVD}
    \State $\begin{bmatrix}
            U_\mathrm{tmp} & S_\mathrm{tmp} & V_\mathrm{tmp}
    \end{bmatrix} = \mathrm{svd}(K)$ \Comment{Perform Local SVD}
\EndIf
\State parallel-bcast($U_\mathrm{tmp},S_\mathrm{tmp},V_\mathrm{tmp}$) \Comment{Broadcast SVD results}
\\
\State $R = \begin{bmatrix}
        V & 0 \\
        0 & \mathrm{eye(b)}
\end{bmatrix}$ \Comment{Prepare V Update}
\State $Q = \begin{bmatrix}
        U & \tilde{P}
\end{bmatrix}$ \Comment{Prepare U Update}
\State $\tilde{Q} = \mathrm{GramSchmidt}(Q)$ \Comment{Necessary?}
\\
\State de-allocate(U,S,V)
\State allocate(U(ny,t),S(t),V(nV+b,l))
\\
\State $S$ = $S_\mathrm{tmp}$(1:l)
\State $V$ = $R$ $V_\mathrm{tmp}$(:,1:l)
\State $U$ = $\tilde{Q}$ $U_\mathrm{tmp}$(:,1:l)

\end{algorithmic}
\end{algorithm}




\begin{algorithm}[H]
\caption{Spatially Parallel / Temporal Serial truncated Principal Component Analysis Algorithm based on a incremental Singular Value Decomposition}
\SetKwInput{KwInput}{Input}                % Set the Input
\SetKwInput{KwOutput}{Output}              % set the Output
\DontPrintSemicolon
  
  %\KwInput{mB-Def, itSVD-rank}
  \KwInput{mB, r}
  \KwOutput{$U \in \mathbb{R}^\mathrm{ny \times r}$, $S \in \mathbb{R}^\mathrm{r}$, $V \in \mathbb{R}^\mathrm{nt, r}$}

  \SetKwFunction{FMain}{Main{\_}SPTS}
  \SetKwFunction{FUpdate}{itSVD{\_}update}
 
  \SetKwProg{Fn}{Function}{:}{\KwRet}
  \Fn{\FMain{}}{
        \tcc{Initialize the (global) itSVD-relevant matrices per processor}
        \textbf{PUBLIC} allocate(U(ny,1),S(1),V(1,1),B(ny,0))\;
        \tcc{Perform the SPTS time integration}
        \For{t=1,nt}
        {
            solve for procedural distributed $1=[1,...,ns]$ instantaneous state variables, Eqn. (a) \;
        	acquire non-dimensionalized state vector y(:), Eqn. (b) \;
        	\tcc{Initialize the itSVD}
        	\eIf{$t=1$}
            {
                $V(1,1) = 1$\;
                $S(1) = y(:)^\mathrm{T} y(:)$,
                $\mathrm{parallel{\_}sum}(S(1)$),
                $S(1) = \sqrt{S(1)}$\;
                $U(:,1) = y/S(1)$\;
                \tcc{Update the bunch matrix B}
            }{
                mB=size(B,2)\;
                allocate(tmp(ny,mB))\;
                tmp(:,:) = B(:,:)\;
                de-allocate(B), allocate(B(ny,mb+1))\;
                B(:,1:mb)=tmp(:,:), B(:,mb+1)=y(:)\;
                de-allocate(tmp), mB=size(B,2)\;
                \tcc{Update the itSVD + clear the bunch matrix B if 1) bunch size reaches pre-defined size or 2) simulation end}
                \If{(mB=mB-Def) \textbf{or} (t=nt)}
                {
                    itSVD{\_}update()\;
                    de-allocate(B), allocate(B(ny,0))\;
                }
            }
        }
        save U, S, V\;
        \KwRet 0\;
  }\;
  
  \tcc{Update the itSVD}
  \SetKwProg{Fn}{Subroutine}{:}{}
  \Fn{\FUpdate{}}{
        $k = \mathrm{size}(U,2)$, $b = \mathrm{size}(B,2)$, $l = \mathrm{min}(r,k+b)$\;
        \tcc{1) $M \in \mathbb{R}^{k \times b}$ 2) Local to Global Operation}
        $M = U^\mathrm{T} B$, parallel-sum($M$)\;
        \tcc{1) $P \in \mathbb{R}^{ny \times b}$ 2) $\tilde{P} \in \mathbb{R}^{ny \times b}$ follows from an Gram-Schmidt based orthonormalization}
        $P = B - U M$, $\tilde{P} = \mathrm{parallel{\_}gram{\_}schmidt}(P)$\;
        \tcc{1) $T \in \mathbb{R}^{b,b}$ 2) Local to Global Operation}
        $T = \tilde{P}^\mathrm{T} P$, parallel-sum($T$)\;
        \tcc{Perform the necessary SVD on one proc only and distribute the data subsequently}
        \If{procID=0}
        {
            $K = \begin{bmatrix}
            S & 0 \\
            0 & T
            \end{bmatrix}$ \;
            $\begin{bmatrix}
            U_\mathrm{tmp}, S_\mathrm{tmp}, V_\mathrm{tmp}
            \end{bmatrix} = \mathrm{svd}(K)$\;
            parallel-bcast($U_\mathrm{tmp},S_\mathrm{tmp},V_\mathrm{tmp}$)
        }
        \tcc{Prepare V Update via old V and identity matrix $I \in \mathbb{R}^{b \times b}$}
        $R = \begin{bmatrix}
        V & 0 \\
        0 & I
        \end{bmatrix}$\;
        \tcc{1) Prepare U Update via old U and P from above 2) Necessary?}
        $Q = \begin{bmatrix}
        U & \tilde{P}
        \end{bmatrix}, \tilde{Q} = \mathrm{parallel{\_}gram{\_}schmidt}(Q)$\;
        \tcc{Increase the U, S, and V sizes (towards the maximum prescribed rank)}
        de-allocate(U,S,V), allocate(U(ny,t),S(t),V(nV+b,l))\;
        \tcc{Finally perform a truncated update}
        $S$ = $S_\mathrm{tmp}$(1:l)\;
        $V$ = $R$ $V_\mathrm{tmp}$(:,1:l)\;
        $U$ = $\tilde{Q}$ $U_\mathrm{tmp}$(:,1:l)
  }
\end{algorithm}



%Die grundlegende Ausgangssituation wird wie folgt angenommen. Ein physikalisches System wird räumlich (womöglich extrem) parallelisiert und anschließend in der Zeit integriert, wobei die physikalische Zeit seriell interpretiert wird. Typisches Beispiele für derartige Räumlich Parallele/Zeitlich Serielle (RPTS) sind quasi unerschöpflich aber vor allem vielfältig in technischen/wissenschaftlichen Anwendungen zu finden. Beispielhaft seien an dieser Stelle das dynamische Verhalten von festen (Struktur) bzw. flüssigen/gasförmigen (Fluid) Kontinua mit möglicherweise untereinander gekoppelter Betrachtung, elektrodynamische Vorgänge oder gar die Modellierung von großskaligen Klimasystemen genannt. BLA BLA BLA

%Generell gehen wir im folgenden davon aus, dass zu einem jeden (diskreten) Zeitpunkt $t$ des (kontinuierlichen) Zeithorizontes $[t^\mathrm{start},t^\mathrm{end}]$ eine Verteilung von beliebig vielen physikalischen Zuständen $y(x_i,t)$ im Anschauungsraum aus einem wie auch immer gearteten, z.B. auf Finiten Differenzen/Volumen/Elemten folgenden, Black-Box-Löser folgt. Für die Anwendungen dieses Papers sind dies beispielsweise die 3 Geschwindigkeitskomponenten $v_i$, der fluiddynamische Druck $p$ und weitere passive/aktive Transportgrößen einer (eulerschen) CFD Simulation.

Die Aneinanderreihung der $s = [1,...,ns]$ Einzelzustandsvektoren $\underline{\varphi}$ gleicher Länge $l = [1,...,nl]$, i.e. gleicher Anzahl räumlicher Freiheitsgrade, erlaubt die Konstruktion eines lokalen Gesamtzustandsvektor $\underline{y}$ der Länge $ny = ns \cdot nl$ zum Zeitpunkt $t \in [1, ..., nt]$ auf Prozessor $p \in [1, ..., np]$, viz.
\begin{align}
    \underline{y}^{(t,p)} =
    \begin{bmatrix}
        \underline{\varphi}^{(1,1:nl,t,p)} \\
        \vdots \\
        \underline{\varphi}^{(ns,1:nl,t,p)}
	\end{bmatrix}
	\qquad \qquad \mathrm{with} \qquad \qquad
    \underline{\varphi}^{(s,1:l,t,p)} =
    \begin{bmatrix}  
		\varphi^{(s,1,t,p)} \\
    	\vdots \\
	    \varphi^{(s,nl,t,p)} 
	\end{bmatrix} \, .
\end{align}
Die Spaltenweise aneinandergereiten Gesamtzustandsvektoren pro Prozesser liefern folgende Möglichkeit zur Definition einer globalen, sich in der Zeit entwickelnden Zustandsmatrix
\begin{align}
    \uuline{Y} = 
    \begin{bmatrix}
            \underline{y}^{(1,1)}   & \cdots    & \underline{y}{(nt,1)} \\
            \vdots                  &           & \vdots                \\
            \underline{y}^{(1,np)}  & \cdots    & \underline{y}^{(nt,np)}
    \end{bmatrix} \label{equ:state_matrix}
\end{align}
der Größe $Y \in \mathbb{R}^{(ny \cdot np) \times nt}$, wobei typischerweise $ny = ns \cdot nl >> nt$ gilt, i.e. die Lösung der betrachteten Probleme sind i.d.R. im Raum deutlich aufwendiger (elliptisch) als in der Zeit und skalieren (nichtlinear) mit der Anzahl der Feldgrößen.
%
Das später gezeigte, maritime Strömungsbeispiel hat beispielsweise $ns = 7$ Feldgrößen bei einer räumlichen Diskretisierung von $nl \approx 10.000$ auf $np \approx 400$ Prozessoren welche über einen Zeithorizont von $nt = 15.000$ Zeitschritten rekonstruiert werden sollen, was eine globale Zustandsmatrix von ungefähr $Y \in \mathbb{R}^{28.000.000 \times 15.000}$ ergibt.
%
Ohne Frage ist es absolut unrealistisch eine Matrix dieser Größenordnung einfach abzuspeichern, weswegen simulationsbegleitendes, ressourcenschonendes PCA Verfahren für die skizzierte Situation vorgestellt wird.

Das zu Grunde liegende Werkzeug ist eine inkrementelle Singulärwertzerlegung. 

%\paragraph{Singular Value Decomposition}
%Angenommen es existiert eine Matrix $\matr{A} \in \mathbb{R}^{N \times M}$, dann lässt sich diese in $d = \mathrm{min}(N,M)$ sortierte, relle Zahlen $s_1 \geq s_2 \geq ... \geq s_d \geq 0$ sowie zwei orthogonale Matrizen $\matr{U} \in \mathbb{R}^{N \times N}$ und $\matr{V} \in \mathbb{R}^{M \times M}$ zerlegen, sodass
%\begin{align}
%\matr{A} = \matr{U} \matr{S} \matr{V}^T
%\quad 
%\quad 
%\mathrm{with}
%\quad 
%\quad 
%\matr{U}^T \matr{U} = \matr{I} \in \mathrm{R}^{N \times N}
%\quad 
%\quad 
%\mathrm{and}
%\quad 
%\quad 
%\matr{V} \matr{V}^T = \matr{I}  \in \mathrm{R}^{M \times M}
%\label{equ:general_svd_definition}
%\end{align}
%gilt, wobei $\matr{S} = \mathrm{diag}(s_1, ..., s_d) \in \mathbb{R}^{d \times d}$ die eindeutigen Singulärwerte auf der Hauptdiagonalen trägt und $\matr{I}$ die Einheitsmatrix darstellt.



\subsection{Truncated Singular Value Decomposition} 
\label{sec:tSVD}
In diesem Fall handelt es sich bereits theoretisch (eine praktische Gleichheit ist numerisch kaum zu realisieren) um eine rank-r Approximation der Matrix $\uuline{A}$, in dem die generelle SVD aus (\ref{equ:general_svd_definition}) in ihrer Größe reduziert wird, viz.
\begin{align}
\uuline{A} \approx \uuline{\tilde{U}} \uuline{\tilde{S}} \uuline{\tilde{V}}^T
\quad 
\quad 
\mathrm{with}
\quad 
\quad 
\uuline{\tilde{U}}^T \uuline{\tilde{U}} = I \in \mathrm{R}^{r \times r}
\quad 
\quad 
\mathrm{and}
\quad 
\quad 
\uuline{\tilde{V}} \uuline{\tilde{V}}^T = I \in \mathrm{R}^{m \times m}
\label{equ:truncated_svd_definition} \, ,
\end{align}
wobei $\uuline{U} \in \mathbb{R}^{n \times r}$, $\uuline{S} = \mathrm{diag}(s_1, ..., s_r) \in \mathbb{R}^{r \times r}$ und $\uuline{V} \in \mathbb{R}^{m \times r}$ nun die tSVD Matrizen reduzierter Größe darstellen. In der Praxis zeigt sich häufig, dass $r << d$ gewählt werden kann, wobei die Qualität der tSVD mit Hilfe des \textit{Eckart-Young-Theorem} durch die vernachlässigten Singulärwerte oder die \textit{Bewahrte Energie der $\eta$ Matrix A} (definiert über die quadrierte Frobenius Norm der Matrix) quantifizierbar ist, viz.
\begin{align}
    ||\uuline{A}  - \uuline{\tilde{U}} \uuline{\tilde{S}} \uuline{\tilde{V}}^T||^2  = \sum_{i=r+1}^{d} s_i^2
    \qquad \qquad
    \mathrm{or}
    \qquad \qquad
    \eta = \frac{||\uuline{\tilde{U}} \uuline{\tilde{S}} \uuline{\tilde{V}}^T||^2}{||\uuline{A}||^2} = \frac{\sum_{i=1}^{r} s_i^2}{\sum_{i=1}^{d} s_i^2} \label{equ:svd_quality_criteria} \, .
\end{align}
Derartige Qualitätskriterien benötigen jedoch die Gesamtheit aller $d$ Singulärwerte, was für technische Anwendungen kaum umsetzbar ist. Es wird daher angenommen das lediglich die ersten $l$ Singulärwerte zur Approximation herangezogen werden können, sosdass $r \leq l \leq d$ gilt, wobei zwar die ersten $r$, aber nicht die alle $d$ Singulärwerte bekannt sind. Hiermit kann das energetische Qualitätskriterium aus Eqn. (\ref{equ:svd_quality_criteria}) abgewandelt werden, in dem eine obere $\eta^\mathrm{u}$ bzw. untere $\eta^\mathrm{l}$ energetische Schranke definiert wird
\begin{align}
    \eta^\mathrm{u} = \frac{\sum_{i=1}^{r} s_i^2}{\sum_{i=1}^{l} s_i^2} 
    \qquad \qquad
    \mathrm{and}
    \qquad \qquad
    \eta^\mathrm{l} = \frac{\sum_{i=1}^{r} s_i^2}{\sum_{i=1}^{l} s_i^2 + (d-l)s_l^2} \, ,
    %\eta^\mathrm{l} = \frac{\sum_{i=1}^{r} s_i^2}{\sum_{i=1}^{l} s_i^2 + \sum_{i=l}^{d} s_i^2} \approx \frac{\sum_{i=1}^{r} s_i^2}{\sum_{i=1}^{l} s_i^2 + (d-l)s_l^2}  \, ,
\end{align}
such that $\eta^\mathrm{l} \leq \eta \leq \eta^\mathrm{u}$ eingehalten wird, wobei die \textit{nicht-bewarte bzw.~vernachlässigte Energie} optimistisch $\eta^\mathrm{neglect} = \sum_{i=l+1}^d s_i^2 \approx (d-l) s_l^2$ abgeschätzt wird.
















The upcoming lines give an introduction to the basic theory of the singular value decomposition (SVD) for real matrices. For this purpose, different variants of the SVD are presented and the for this paper relevant properties are summarized.
%
The following statements are standard information and are reproduced for completeness and, above all, for the sake of understanding; their proofs are assumed to be known.
%
\begin{theorem}[Singular Value Decomposition (SVD)]
\label{def:SVD}
Let $\matr{A} \in \mathbb{R}^{N \times M}$. Then there exist the orthogonal matrices $\matr{U} = \left( \vect{u}_1, ..., \vect{u}_N \right) \in \mathbb{R}^{N \times N}$ and $\matr{V} = \left( \vect{v}_1, ..., \vect{v}_N \right) \in \mathbb{R}^{M \times M}$ as well as a diagonal matrix $\matr{S} = \left( s_i \delta_{ij} \right)_{ij} \in \mathbb{R}^{N \times M}$ such that
\begin{align}
    \matr{A} = \matr{U} \matr{S} \matr{V}^T = \sum_{i=1}^d s_i \vect{u}_i \vect{v}_i^\mathrm{T}
\end{align}
with unique singular values $s_1 \geq ... \geq s_d \geq 0$, singular vectors $\vect{u}_i, \vect{v}_j$ and $d = \mathrm{min}(N, M)$.
\end{theorem}
%
Note that the theoretical equality $\matr{A} = \matr{U} \matr{S} \matr{V}^T$ holds only in the absence of numerical rounding errors, which is not necessarily feasible for practical applications with very large matrices. Based on the preceding, two remarks of particular emphasis follow, which relate to the norm of the matrix $\matr{A}$ to be approximated as well as to its rank.
%
\begin{corollary}
\label{cor:norms}
Let $\matr{A} \in \mathbb{R}^{N \times M}$. Then the invariant $||\matr{A}|| = ||\matr{S}||$ yields
\begin{enumerate}
    \item $||\matr{A}||_2 = s_1$
    \item $||\matr{A}||_F = \sqrt{\sum_{i=1}^N \sum_{i=1}^M |a_{ij}|^2} = \sqrt{\sum_{i=1}^d s_i^2}$
\end{enumerate}
where $||\cdot||_2$ and $||\cdot||_F$ refer to the L2 and Frobenius norm, respectively.
\end{corollary}
%
\begin{corollary}
\label{cor:rank}
Let $\matr{A} \in \mathbb{R}^{N \times M}$ with corresponding SVD $\matr{A} = \matr{U} \matr{S} \matr{V}^\mathrm{T}$, $\matr{U} = \left( \vect{u}_1, ..., \vect{u}_N \right) \in \mathbb{R}^{N \times N}$, $\matr{V} = \left( \vect{v}_1, ..., \vect{v}_M \right) \in \mathbb{R}^{M \times M}$ and $r = \mathrm{max}(k \in \mathbb{N}: s_k \neq 0)$ the amount of positive singular values. Then
\begin{enumerate}
    \item $\mathrm{rank}(\matr{A}) = r$
    \item $\matr{A} = \sum_{i=1}^r s_i \vect{u}_i \vect{v}_i^\mathrm{T}$
\end{enumerate}
hold.
\end{corollary}
%
Thus Cor. \ref{cor:rank} yields that only the first $r$ singular vectors are needed to determine the matrix $\matr{A}$ via the SVD which in turn allows for the following definition of a reduced SVD.
%
\begin{definition}[Reduced Singular Value Decomposition (rSVD)]
\label{def:rSVD}
Let $\matr{A} \in \mathbb{R}^{N \times M}$ with $\mathrm{rank}(\matr{A}) = r \leq \mathrm{min}(N,M)$. Then there exist the orthogonal matrices $\matr{U}_r = \left( \vect{u}_1, ..., \vect{u}_r \right) \in \mathbb{R}^{N \times r}$ and $\matr{V}_r = \left( \vect{v}_1, ..., \vect{v}_r \right) \in \mathbb{R}^{M \times r}$ as well as a diagonal matrix $\matr{S}_r = \left( s_i \delta_{ij} \right)_{ij} \in \mathbb{R}^{r \times r}$ such that
\begin{align}
    \matr{A} = \matr{U}_r \matr{S}_r \matr{V}_r^T = \sum_{i=1}^r s_i \vect{u}_i \vect{v}_i^\mathrm{T}
\end{align}
with unique singular values $s_1 \geq ... \geq s_r \geq 0$ and singular vectors $\vect{u}_i, \vect{v}_j$.
\end{definition}
%
The methodology of neglecting zero-valued singular values inspires the approximation approach of additionally truncating the smallest non-zero singular values. This represents the assumption that small singular values have only a minor impact on the approximation quality leading to the definition of a truncated SVD.
%
\nkuehl{t is already used for the physical time ...}
\begin{definition}[Truncated Singular Value Decomposition (tSVD)]
\label{def:tSVD}
Let $\matr{A} \in \mathbb{R}^{N \times M}$ with $\mathrm{rank}(\matr{A}) = r$ and corresponding rSVD $\matr{A} = \matr{U}_r \matr{S}_r \matr{V}_r^T $. Then the rank-r tSVD of $\matr{A}$ with $0 < t < r$ is defined as
\begin{align}
    \matr{A}_t = \matr{U}_t \matr{S}_t \matr{V}_t^T = \sum_{i=1}^t s_i \vect{u}_i \vect{v}_i^\mathrm{T}
\end{align}
with $\matr{U}_t = \left( \vect{u}_1, ..., \vect{u}_t \right) \in \mathbb{R}^{N \times t}$, $\matr{V}_t = \left( \vect{v}_1, ..., \vect{v}_t \right) \in \mathbb{R}^{M \times t}$ and $\matr{S}_t = \mathrm{diag}(s_1, ..., s_t) \in \mathbb{R}^{t \times t}$. Thereby $\matr{A}_t \in \mathbb{R}^{N \times M}$ denotes the matrix obtained by neglecting the $r-t$ smallest singular values of $\matr{A}$ in its rSVD.
\end{definition}
%
For the choice of the reduced order $r$ there is no clear way to determine it a-priori, i.e. before approximation starts. The overall goal is almost always to choose a $t$ as large as possible and as small as necessary so that $\matr{A}_t \approx \matr{A}$. The above truncation in terms of a tSVD raises the question on the impact of the truncation to the overall approximation quality and leads to the following theorem that goes back to ... .
%
\begin{theorem}[Eckart-Young Theorem]
\label{the:eckart_young}
Let $\matr{A} \in \mathbb{R}^{N \times M}$ with $\mathrm{rank}(A) = r$ and $\matr{A}_t \in \mathbb{R}^{N \times M}$ obtained by the rank-t SVD of $\matr{A}$ with $0 < t < r$. Then
\begin{align}
    ||\matr{A} - \matr{A}_t|| = 
    \left\{
        \begin{array}{ll}
            s_{t+1} & \mathrm{if~} ||\cdot||_2 \\
            \sqrt{\sum_{i=t+1}^r s_i^2} & \mathrm{if~} ||\cdot||_F \\
        \end{array}
    \right.
\end{align}
holds. Here $s_{t+1}$ denotes the largest singular value of $\matr{A}$ which is no singular value of $\matr{A}_t$. \nkuehl{Input von HF, stimmt das?}
\end{theorem}
%
Instead of subtracting the matrices $\matr{A}$ and $\matr{A}_t$ from each other first and then considering the absolute error ($\to 0$), another approximation quality measure follows from first applying a norm to each matrix respectively and subsequently consider a relative error (here $\to 1$). In this context the so-called "energy" of a matrix is employed, which --of course-- has no physical energetic character, but is typically defined via the squared Frobenius norm of the matrix, cf. Cor. \ref{cor:norms} and one is usually interest in the retained energy of the approximation.
%
\begin{definition}[Retained Energy]
\label{def:SVD_energy}
A criterion for the quality of the truncation of the tSVD is the retained energy of the approximation. Since the energy of a matrix A is definded via its squared Frobenius norm ($|| \cdot ||_F^2$) the retained energy is given by
\begin{align}
    \eta^r = \frac{||\matr{A}_t||_F^2}{||\matr{A}||_F^2} = \frac{\sum_{i=1}^t s_i^2}{\sum_{i=1}^r s_i^2} \label{equ:SVD_energy}
\end{align}
where $t < r$ denotes the rank of the tSVD and r the rank of $\matr{A}$.
\end{definition}
%
However, such quality criteria require the totality of all $d$ singular values, which is hardly feasible for technical applications. Therefore, it is assumed that only the first $l$ singular values are available for the approximation, so that $r \geq l \geq t$ is valid, where the first $l$, but not all $d$ singular values are known and the rank $r$ is roughly available (e.g. via the maximum number of time steps used for the SVD). Hereby, the energetic quality criterion (\ref{equ:SVD_energy}) can be modified, so that an upper $\eta^\mathrm{u}$ and lower $\eta^\mathrm{l}$ energetic bound is defined.
%
\begin{definition}[Retained Energy Limits]
\label{def:SVD_energy_limits}
Since the calculation of all singular values $s_i$ of a matrix $\matr{A}$ in Def. \ref{def:tSVD} is impractical for large matrices, the following bounds are introduced. Let $r \geq l \geq t$ be the amount of economically computable singular values. Then an upper bound is given by
\begin{align}
    \eta^u = \frac{\sum_{i=1}^t s_i^2}{\sum_{i=1}^l s_i^2}
\end{align}
and a lower bound by
\begin{align}
    \eta^l = \frac{\sum_{i=1}^t s_i^2}{\sum_{i=1}^l s_i^2 + (r-l)s_l^2}
\end{align}
such that $\eta^l \leq \eta \leq \eta^u$ holds.
\end{definition}
Here, the \textit{non-maintained or neglected energy} is optimistically estimated, viz. $\eta^\mathrm{n} = \sum_{i=l+1}^r s_i^2 \approx (r-l) s_l^2$.
